Placement Laundering and the Complexities of Attribution in Online Advertising

A basic assumption in online advertising is that it is possible to attribute a view of a particular ad creative (i.e., an impression) to a particular web page. In practice, however, the seemingly simple task of ad attribution is challenging due to the scale, complexity and diversity of ad delivery systems. In this paper, we describe a new form of fraud that we call placement laundering, which exploits vulnerabilities in attribution mechanisms. Placement laundering allows malicious actors to inflate revenue by making ad calls that appear to originate from high quality publishers. We describe the basic aspects of placement laundering and give details of two instances found in the wild. One of the instances that we describe abuses the intended functionality of the widely-deployed SafeFrame environment. We describe a placement laundering detection method that is capable of identifying a general class of laundering schemes, and provide results on tests with that method.

==> bimage.tex <==
\subsection{Bimage}
% overview
This instance of placement laundering employs a highly complex method of ad delivery.  The techniques used include ephemeral URLs,  strong encryption, heavily obfuscated javascript code and metaprogramming to execute video ad delivery.  Additionally this example exhibits scalability, durability and adaptability over time. 

The URL that ultimately returns a video ad to a browser is human-readable and suggests innocuous content. Several example domains are {\tt\url{loansaver.com}} and {\tt\url{trainsandplaneshobbies.com}}. Telemetry that accompanies a video ad that happened to be delivered in this manner will indicate that the ad was displayed alongside human-readable content on a family-friendly publisher's page.  See Figure \ref{fig:ads-stream-net-human-readable-referer-2}.  However, in early 2016, we associated between 2\% and 5\% of ads served on these domains with ad networks that cater to adult content. A followup review of panelist traffic during November of 2016 confirmed this. This is an issue called {\em brand safety}. 


% We initially discovered this instance during a review of video ad campaign traffic within panelist data~\footnote{Video ads typically pay much higher CPMs than display ads.}. 
% Several domains were credited with very large impression volume yet were literally inaccessible from search engine results ({\em i.e.,} cloaked sites - details below). 
During late 2015, this scheme was associated with hundreds\footnote{A partial list: www.wealthscreen.com, www.carsluxurious.com, www.lastwordedits.com, www.thatspoon.com, www.homescelebrity.com, www.jewelryboxhome.com, www.precisionmoney.com, www.athletetribune.com, www.womensthread.com, www.readysetpaint.com, www.craftschest.com, www.hobbyattraction.com, www.loanssaver.com, www.legendsbeauty.com, www.trainsandplaneshobbies.com, www.familyglass.com} of distinct domains.  We observed about five domains in service any point in time. We also observed that the set of highly-active domains changes regularly.  Daily impression volume varies, ranging from 200k video impressions on active domains per day 
 %during mid-2014 
 to over 1M video impressions per day.
 %in early 2015.   
 There are also dozens of ad servers whose purpose appears solely dedicated to the delivery of ads on these domains. Given the intricate, complex flow of traffic involved in each ad delivery, we believe that the ad servers and these domains are simply different parts of the same operation.  
%Tracking the activity here involves a semi-automated process of continual monitoring.  
The nickname {\em bimage} is derived from the URL path of the iframes that contain these ads~\footnote{In early 2014, a news story (http://adage.com/article/digital/ad-fraud-operation-fools-detection-companies-nets-millions/293929/) associated several domains related to those described here with ad fraud.}.

Most of these domains are simply not accessible from search engine results. This is highly unusual for a publisher who wishes to earn ad revenue from organic human traffic.  Yet the following lines of Javascript code are common to many of the identified domains. The code redirects a web browser to an error page if the page referrer does 
not contain the string ``\mbox{monkeysee}'':
\begin{verbatim}
if (g.indexOf("monkeysee")==-1 && f != g){
 return c.RefererSecurityBreached=!0, 
  d=!0, 
  window.location = 
   "http://{0}/referror?{1}".format(f, b), 
  !0
}
\end{verbatim}
The consequence is that if a user attempts to reach one of these domains from a set of search engine results, the page renders an error.

Another unusual feature is that many of these domains display fake ads.  This is not obvious from a cursory visual inspection.  Indeed, the creatives are sometimes from well-known brands and recent ad campaigns.  Clicks on these ad creatives send a user to an appropriate landing page ({\em e.g.}~the landing page for a Tide creative is Tide.com). But no tracking occurs.  The links are simply direct HTML links to brand home pages.  It seems clear that this is done to make the target sites appear to be legitimate.  Furthermore, the content on each site is related to whatever the domain name suggests. For example, {\tt\url{carsluxurious.com}} hosts stories and photos of fancy cars. 

%None of the sites have brand safety problems or host anything that might draw undue attention.
%% Standard telemetry (e.g. referrer or 
%% window location) would also offer no insight into the fact that the ad
%% was hosted in an iframe.

% In addition to the hundreds of ``publisher" domains just described, dozens of ad servers are associated with video delivery and distribute traffic among the content sites. An incomplete list of these ad servers is 'ads-stream.net', 'ads-cast.com', 'ads-safe.net', 'ads-switch.com', and "eloquentads.net'. Inspection of URLs in panel traces occasionally reveals names of ad servers which do not resolve to IP addresses. We believe there is a fallback mechanism so that if an ad server fails to resolve, a working ad server is used. 

%In early 2014, a news story\footnote{http://adage.com/article/digital/ad-fraud-operation-fools-detection-companies-nets-millions/293929/} associated several domains related to those described here with ad fraud. Subsequent to that story, we witnessed the ad delivery mechanism change to pass information through cookies instead of query strings.

% The significance of this change is that information is passed in an HTTP header, not in the URL and therefore characteristic strings  associated with this scheme are less visible to standard methods of traffic measurement.  
Figure \ref{fig:http-transaction-headers} describes the sequence of messages sent between a web browser and the relevant web servers.
This sequence has two significant features: it updates the user's browser by placing cookies on it and it updates the web servers by creating URLs that expire after a few minutes.
Without the proper cookie, an ad will not render. As a result, even if a person is able see a complete sequence of URLs associated with an ad call, that person will not be able to reconstruct the steps required to witness a video ad. Instead, the user will enconter a 404-not found page, a non-monetized ad in a bimage.aspx page or the publisher's ``content'' site.  

\begin{figure}[tp]
\includegraphics[width=5.00in]{images/http-transaction-headers.pdf}
\caption{This figure traces the complex sequence of calls involved in the delivery of a single ad in the bimage example. 
	Both client and server state are updated: the intermediate GET requests 
	signal the servers to build  ephemeral URLs which host 
	the final iframe that displays the video player.  The last URL in the sequence
	appears to host human-readable content.  But the page actually just displays a video ad.
	The referrer fields of the final page show gardendsdecor.com. The unusual mechanism and 
	observed traffic characteristics lead us to believe that
	the ad servers and the publishers are two parts of the same operation.
	% The initial call is'ads-switch.com/rt?id=5&k=cwoTr2gWTGZw2rr0g&pub_id=174'
	}
\label{fig:http-transaction-headers}
\end{figure}
%  \begin{small}
%  \begin{verbatim}
%  GET: 'http://ads-switch.com/rt?id=5&\
%        k=nxRiNOF0P6f74Kw&pub_id=174'
%  RESPONSE HEADER:
%    HTTP/1.1 302 Found
%    ...
%    Location: http://ads-switch.com/r1?...\
%        uri=ingardens.com...\
%        sb%2526query%253dmU3l.bxklMo...
%    Set-Cookie: PREF_RC_R5=... 
%  
%  GET: 'http://ads-switch.com/r1?...\
%        uri=ingardens.com...\
%        sb%2526query%253dmU3l.bxklMo...'
%  RESPONSE HEADER:
%    HTTP/1.1 302 Found
%    ...
%    Location: http://ingardens.com/rc?dt=...
%  
%  GET: 'http://ingardens.com/rc?dt=...'
%  RESPONSE HEADER:
%    HTTP/1.1 302 Found
%    ...
%    Location: http://ads-verify.net?\
%        tt=sb&query=mU3l.bxklMon...
%    Set-Cookie: PREF_LC=FpWk.DD16pc7...\
%        domain=.ingardens.com; ...
%  
%  GET: 'http://ads-verify.net?\
%        tt=sb&query=mU3l.bxklMon...
%  RESPONSE BODY:
%    ...
%    <iframe src="http://ads-switch.com/...>
%    ...
%    </iframe>
%    ...
%  \end{verbatim}
%  \end{small}
% The innermost call to ads-switch.com eventually refreshes the top-level page
% with an ad call to a page which appears to host content when in fact it
% hosts a video ad.


 %Delivery of the video ad involves loading of the strong-encryption library, crypto.js.  We are unaware of any other instances where crypto.js loads during the course of ad delivery.

%We said earlier that the video player code is hosted at a short-lived URL. Strictly speaking, this isn't true. When the URL expires, a lightweight dummy player is returned. 
%The live URL returns a player with a code-base that is twice the size of the dummy player.
% 
% The url for the page looks like:
% \begin{small}
% \begin{verbatim}
% http://..../vidmanager.min.js?q=1E5...Slq8-
% \end{verbatim}
% \end{small}
%
Finally, the ad's video player code is obfuscated in an unusual way.  The video player code returns a function which, in order to run, accepts arguments that are derived from the web browser's cookie and the page URL.  The function appears to generate a string of javascript which, after several rounds of deobfuscation, is executed with a call to \texttt{eval()}.  This call, in turn, creates several anonymous Javascript functions which load a video player in the browser. The starting and ending portions of the Javascript video player code are:
\begin{small}
\begin{verbatim}
var J5L=(function f(o,s){var j='',
  E=unescape('%13%1E*L*%246%01%08f%5...
       <skip 150k bytes> 
    ...FI%11%02"), "liOu...qrFIfrOjgT")());
\end{verbatim}
\end{small}
This video player is hosted at a short-lived URL. When the ephemeral URL expires, a lightweight dummy player is returned instead.
The ``real'' URL returns a player with a code-base that is approximately twice the size (in bytes) of the dummy player. 

\begin{figure}[tp]
\hspace{-0.0625in}\includegraphics[width=4.25in]{images/ads-stream-net-human-readable-referer-zoom-edits}
\caption{% After the ad is served, the ad-hosting iframe loads one of the 
	% template domains which shows up as the referrer to all 
	% items within it.  This is referer appears to host content.  The
	This screen capture, related to the bimage scheme, shows a video loading underneath an ad hosted on \url{adserver0.net}. The HTTP Referer field of the innermost iframe is set to a URL that concerns home repair projects. The domain \url{greeneryblog.com} and the story concerning home repair were not loaded by the user during the sequence of events that resulted in this impression delivery. What is visible here would normally render within an iframe on a third party publisher's page. A portion of traffic related to this scheme displayed video ads on domains that serve adult content.}
\label{fig:ads-stream-net-human-readable-referer-2}
\end{figure}

% detection/mitigation
%The scale and adaptability of the infrastructure means that a straightforward blacklist-based approach is not likely to be effective. Additionally, the domains that we know of are hosted on a wide variety of services. Thus a reverse-lookup of domains on blacklisted IPs is also likely to be ineffective.

% The discovery of this was found via customized ad telemetry associated with 
% video ad providers and deployed as part of an experimetal javascript tag.  
% Subsequent audits of comScore telemetry (panel, cat and census data) confirmed
% outlier affinity of several of these domains with video ad providers. 


==> emulse.tex <==
\subsection{Emulse}
This scheme effectively mimics a legitimate ad-serving scenario. As noted in Section~\ref{sec:background} publishers often create URLs that are hosted on their own domains that are dedicated exclusively to generating ad requests and displaying ads. Typically the content of these URLs renders within a sandboxed iframe. The primary reason for this is that code within such an iframe is limited in functionality. In particular, the publisher's primary content is protected from malicious third-party code that could, for example, inject or delete content or even interfere with the user's experience.  These URLs usually "self-identify" by having paths that describe viewport size or describe some other attributes that are relevant to the ad serving process.  Placement laundering can occur when the publisher's self-identifying URL is rendered on a different publisher's page.  

% As in the  {\tt\url{glamwomen.com}} case, in the event that an ad is not served to the web client, the fallback mechanism simply loads the domain's front page inside the iframe.  The effect of this fallback is to inflate the visitor count to the publisher's site.  This effectively increases the publisher's reputation.  

Two domains involved in this example are \mbox{\tt\url{mensstylebook.com}} and \mbox{\tt\url{highspeedtesting.com}}\footnote{As of November 2016, neither \mbox{\tt\url{mensstylebook.com}} nor \mbox{\tt\url{highspeedtesting.com}} are maintained. They are partially preserved at the web archive URL, \mbox{\tt\url{http://web.archive.org/web/20160121082313/http://mensstylebook.com/}}.}.  Both domains host genuine content and the publisher does attempt to court an audience that will see display ads when they visit the sites. Campaign telemetry reported that ads are served on self-advertising URLs with paths similar to \texttt{/adserver/2/160x600.php}.  However, neither domain uses this dedicated ad-serving path to serve ads on itself. Instead, the publisher's in-house ad exchange was used as the public-facing mechanism. In fact, the screen capture of Figure~\ref{fig:watch-series-to-highspeedtesting-emulse-mensstylebook-zoom-edits} shows an instance where the \mbox{\tt\url{mensstylebook.com}} iframe nests in {\tt\url{highspeedtesting.com}} and neither domain bears any relationship with the publisher whose URL appears in the browser location bar.

A unique feature of this instance is the use of the HTTP POST method\footnote{\texttt{curl -vvv -X POST -d"mn=666" 'mensstylebook.com/adserver/2/160x600.php'}} as part of the ad call sequence.  The response to the POST request is a redirect to a URL hosted on \mbox{\tt\url{emulse.com}}. This, in turn, redirects the browser to one of the domains {\tt\url{highspeedtesting.com}} or {\tt\url{mensstylebook.com}}. The body of the POST request is unavailable to web-based telemetry so it is impossible to reconstruct ad calls from telemetry alone.  This thwarts standard attribution techniques that rely on standard methods of telemetry such as HTTP referer and JavaScript location information.  We relied on panelist data to reconstruct and replicate the necessary sequence of HTTP calls. 


% This example was discovered as part of the exploration of URL structure that was described in the previous section. Although the URLs are clearly related to hosting ads, two features were unusual. First, we noticed the pairing of \url{highspeedtesting.com} and \url{mensstylebook.com} in panelist activity. Second, we observed the identical URL structure of these sites. 
A web search seeking additional information about these domains returned a security blog post hosted on {\tt\url{fireeye.com}} entitled "Ads Gone Bad"\cite{adsgonebad}.  The observed volume of panelist traffic attributed to the domains in this instance is 3K per day. 
% FIXME - add a sentence or two on how we discovered this threat and which data sources were used - similar to the last paragraph on Adhexa.  Also be clear about how money is made.

%%    FIXME
%%    %% Characteristics: mensstylebook
%%    %% -----------------------------
%%    %% Unifying mensstylebook: emulse.com
%%    %% comscore=> SELECT  url_refer_host,COUNT(*) AS ccc FROM panel.panel_fact WHERE recorded >= '2015-05-27' AND recorded < '2015-05-28' AND  domain_name = 'emulse.com' GROUP BY url_refer_host ORDER BY ccc DESC;
%%    %% -[ RECORD 1 ]--+---------------------
%%    %% url_refer_host | mensstylebook.com
%%    %% ccc            | 1155
%%    %% -[ RECORD 2 ]--+---------------------
%%    %% url_refer_host | highspeedtesting.com
%%    %% ccc            | 889
%%    %% -[ RECORD 3 ]--+---------------------
%%    %% url_refer_host | creative.emulse.com
%%    %% ccc            | 208
%%    %% 
%%    %% One panelist active on mensstylebook.com without any corresponding content visits:
%%    %% comscore=> SELECT *  FROM panel.panel_fact WHERE recorded >= '2015-05-27' AND recorded < '2015-05-28' AND machine_id = 182648158 ORDER BY recorded;
%%    %% 30 minutes of activity on a panelist:
%%    There are legitimate reasons and instances where an ad server hosts iframes, has built-out 
%%    infrastructure for delivering/hosting ads on the page. However, mensstylebook.com and
%%    highspeedtesting.com do not deploy their ad hosting service on their page.
%%    A partial trace of a single panelist's visit to mensstylebook.com is below 
%%    It shows 30-second refreshes with occasional random loads 
%%    of "content" pages.  The trace continues this way for 
%%    30 minutes. Each call represents an attempt to load 
%%    an ad or invocation of a fallback mechanism to load the primary 
%%    publisher page.
%%    
%%    Since the site doubles as a publisher, there is a fallback mechanism which
%%    occasionally is invoked when an ad fails to place, namely 
%%    the full page loads in the iframe. Publisher
%%    telemetry then loads, potentially offering "credit"
%%    for a page view when in fact no page loaded.
%%    
%%    %% comscore=> SELECT recorded,query_string  FROM panel.panel_fact WHERE recorded >= '2015-05-27' AND recorded < '2015-05-28' AND machine_id = 182648158 AND domain_name = 'mensstylebook.com' ORDER BY recorded;
%%    \begin{small}
%%    \begin{verbatim}
%%    time     mensstylebook.com path
%%    ---------------------------------
%%    11:30:01 /adserver/2/160xx600.php
%%    11:30:02 /adserver/2/160xx600.php?mn=666
%%    11:30:02 /adserver/2/160x600.php?mn=666
%%    11:30:02 /adserver/2/160x600.php
%%    11:30:10 /fashion/fashion-guide-for-men-in-their-40s/
%%    11:30:10 /adserver/2/160xx600.php?mn=666
%%    11:30:11 /?random
%%    11:30:11 /adserver/2/160xx600.php
%%    11:30:12 /adserver/2/160x600.php?mn=666
%%    ...
%%    \end{verbatim}
%%    \end{small}
%%    Many of these urls are interstitial. Only a small
%%    subset render ads. Similar to the example above, javascript is returned to 
%%    write a POST submission to the document, with
%%    appropriate commands. If well-formed 
%%    commands are issued, the server eventually sends a 
%%    request to creative.emulse.com which (after several more redirects
%%    through emulse and mensstylebook.com) loads a VPAID tag and 
%%    other data for rendering video ads. The specific form 
%%    of these URLs (e.g. adserver, 160x600, etc.) could 
%%    be easily replaced by the operators of this site with urls that host other
%%    content on the publisher which switch to Ad delivery mode as in the
%%    example above.
%%    
%%    The POST method leverages hidden forms to upload data, and while different
%%    in form, expresses the same basic idea as shown above:
%%    \begin{small}
%%    \begin{verbatim}
%%    <form \
%%        action='http://mensstylebook.com/.../160xx600.php' \
%%        method='POST' id='form1'>
%%     <input type='hidden' name='mn' value='666'>
%%    </form>
%%    <script language='JavaScript'>
%%      document.getElementById('form1').submit();
%%    </script>
%%    \end{verbatim}
%%    \end{small}
% this is the acual ad call
% curl -vvv -X POST -d"mn=666" 'mensstylebook.com/adserver/2/160x600.php'
%% from the client  (see source comments)
%% Jeff-Kline-MBP:paper jeffkline$ curl -vvv 'mensstylebook.com/adserver/2/160xx600.php'
%% *   Trying 162.247.49.242...
%% * Connected to mensstylebook.com (162.247.49.242) port 80 (#0)
%% > GET /adserver/2/160xx600.php HTTP/1.1
%% > Host: mensstylebook.com
%% > User-Agent: curl/7.42.1
%% > Accept: */*
%% > 
%% < HTTP/1.1 302 Moved Temporarily
%% < Server: nginx
%% < Date: Wed, 03 Jun 2015 22:45:48 GMT
%% < Content-Type: text/html; charset=UTF-8
%% < Transfer-Encoding: chunked
%% < Connection: keep-alive
%% < X-Powered-By: PHP/5.6.8
%% < Location: http://mensstylebook.com
%% < 
%% * Connection #0 to host mensstylebook.com left intact
%% Jeff-Kline-MBP:paper jeffkline$ curl -vvv 'mensstylebook.com/adserver/2/160xx600.php?mn=666'
%% *   Trying 162.247.49.242...
%% * Connected to mensstylebook.com (162.247.49.242) port 80 (#0)
%% > GET /adserver/2/160xx600.php?mn=666 HTTP/1.1
%% > Host: mensstylebook.com
%% > User-Agent: curl/7.42.1
%% > Accept: */*
%% > 
%% < HTTP/1.1 200 OK
%% < Server: nginx
%% < Date: Wed, 03 Jun 2015 22:45:56 GMT
%% < Content-Type: text/html; charset=UTF-8
%% < Transfer-Encoding: chunked
%% < Connection: keep-alive
%% < X-Powered-By: PHP/5.6.8
%% < 
%% <html>
%%               <head></head>
%%               <body>
%%               <form action='http://mensstylebook.com/adserver/2/160xx600.php' method='POST' id='form1'>
%%               <input type='hidden' name='mn' value='666'>
%%               </form>
%%               <script language='JavaScript'>document.getElementById('form1').submit();</script>
%%               </body>
%% * Connection #0 to host mensstylebook.com left intact
%%               </html>
%% 

%%%%   The itermediary for mensstylebook has an fallback mechanism when attempts to display an ad fail.
%%%%   It calls emulse.com with a special query string which returns a body with a META refresh tag, with the 
%%%%   target seemingly chosen at random:
%%%%   \begin{small}
%%%%   \begin{verbatim}
%%%%   GET: 'https://emulse.com/?g/XZ2NSPT'
%%%%   <META HTTP-EQUIV="refresh" CONTENT="0; \
%%%%       URL=http://mensstylebook.com/?random">
%%%%   
%%%%   GET: 'https://emulse.com/?g/XZ2NSPT'
%%%%   <META HTTP-EQUIV="refresh" CONTENT="0; \
%%%%       URL=http://httpurl.blogspot.com/?...">
%%%%   
%%%%   GET: 'https://emulse.com/?g/XZ2NSPT'
%%%%   <META HTTP-EQUIV="refresh" CONTENT="0; \
%%%%       URL=http://www.google.com/....\
%%%%         q=beyonce+the+new+mom...\
%%%%         url=http%3A%2F%2Fmensstylebook.com/\
%%%%           women/beyonce-the-new-mom...">
%%%%   \end{verbatim}
%%%%   \end{small}
%%%%   The google query returns a javascript redirect in the body.

%% The query to google returns a redirect to mensstylebook. This has 
%% several potential benefits to audience measurment on mensstylebook, including apparent organic searches
%% and google referrer strings.
%%                                    --(success)-> ad display in mensstylebook iframe
%% 				 /
%%  incoming -> emulse (intermediate) 
%% 				 \ 
%% 				   --(fail)-> google, blogspot, mensstylebook content
%% 
%% This fallback mechasm may be used in two possible ways. The image 
%% (./data/mode/mensstylebook.com_sellmall.info_connection.png )
%% shows a referer field clearly set to mensstylebook content url. The theory for this is that 
%% the traffic went through emulse -> mensstylebook which issued a queiry to run an ad. When the ad
%% was placed, mensstylebook returned a string that redirected to sellmall.info which then displayed the ad.
%% 
%% There is a similar fallback image showing in bimage (attainliving)

%%%% A hosting web site with iframes dedicated to ads.  This is, quite common and offers
%%%% security benefits.  Publisher bluffing referrer fields.
%%%% The result is that telemetry on mensstyle book appears to be getting 
%%%% SEO content or diverse referrer traffic while in reality it was driven by a failed attempt to
%%%% place an ad. 
% (see ./data/mode/mensstylebook.com_google_redirect_fallback.png)
%% 
%% Characteristics: highspeedtesting
%% ---------------------------------
%%     The image 
\begin{figure}[tp]
\includegraphics[width=4.25in]{images/watch-series-to-highspeedtesting-emulse-mensstylebook-zoom-edits}
\caption{The browser location bar displays the publisher watch-series-tv.to. This publisher loads the sequence of nested iframes highspeedtesting.com $\rightarrow$ emulse.com $\rightarrow$ mensstylebook.com $\rightarrow$ emulse.com $\rightarrow$ messtylebook.com. The video ad impression is attributed to mensstylebook.com. }
\label{fig:watch-series-to-highspeedtesting-emulse-mensstylebook-zoom-edits}
\end{figure}
%%%%  shows the relationship of some generic ad server infrastructure to highspeedtesting 
%%%%  making calls through emulse to mensstylebook. This is a consistent 
%%%%  feature of this set of URLs, and the structure of URL suggests shared code base.

%% The url structure of mensstylebook and highspeedtesting and several other 
%% (now defunct) sites all share similar traits, namely
%% 
%% As one illustration of how important the query parameters are:
%% A call to 
%% 	http://mensstylebook.com/adserver/2/728xx90.php?mn=666
%% returns a splot for an ad while this:
%% 	http://mensstylebook.com/adserver/2/728xx90.php
%% redirects to the top-level page of mensstylebook.
%% 
%% highspeedtesting.com/adserver/ads03/160.php?mn=8

%%%%   Evolution over time: the urls described on the fireeyeblog fail to resolve, we also
%%%%   observed decrease in traffic.

% Just prior to shutdown, quickmensguide.com was briefly a phishing site just prior to going offline. This 
% is documented in the wayback machine.  Ironicly, the owner of quickmensguide.com is owner of of the domain 
% no-phishing.org (wjones@wwwpromoter.com). 
%% This domain name is registered to wwwpromoter, also the owner of hometechproducts. Both quickmensguide and hometechproducts 
%% are Mode Media affiliates (./data/mode/quickmensguide_brash_connection.png,./data/mode/hometechproducts_brash_site.png).
%% The home office of wwwpromoter.com is a virtual office in downtown Manhattan.


==> glamwomen.tex <==
\subsection{Glamwomen}
% FIXME
% The adserver roimediadigital.com is anonymously-owned. It
% serves thousands of ads, primarly to three domains:
% glamwomen.com, quickcookingguide.com and tripandleisure.com. These three domains 
% are associated with other "live" domains though these other 
% domains do not appear to be actively engaged in ad serving.
% FIXME: Figure \ref{fig:adhex-glamwomen-census} shows glamwomen.com ad
% hosted within a third party domain, the referring URL appears 
% to host content related to workout songs.
In this instance, the publisher maintains a public-facing and innocuous ``staging'' URL whose purpose is to redirect traffic to a secondary URL also maintained by the publisher. The secondary URL delivers an ad to a browser only if the Referer in the HTTP request matches the staging URL.  If the Referer does not match, the secondary URL returns the default page content. 

Figure \ref{fig:glam_ref} has a visual representation showing the sequence of events. The staging URL is \mbox{\tt\url{http://glamwomen.com/featured?category=4}}. The secondary URL is \mbox{\tt\url{http://glamwomen.com/living/make-this-super-easy-diy-string-ball-home-decor}}.  
As the text within the URL suggests, the default content describes a do-it-yourself (DIY) home decorating project. In the event that the publisher domain is disabled or blacklisted, a domain with a clean reputation may be put into service quickly.
% Figure~\ref{fig:adhex-glamwomen-census} shows how this can be misleading.

% This example was discovered while exploring the content and structure of URLs returned by ad campaign telemetry.  During the exploration, we observed that many advertisements attributed to a publisher (glamwomen.com) appeared to render alongside page content. This is a highly unusual design choice by a publisher. Manual review of the site and investigation of panelist data explained what was happening.

\begin{figure}[tp]
\centering
\includegraphics[height=2.75in]{images/glamwomen-referer-keynote}
% \includegraphics[height=1.75in]{images/glamwomen-referer}\vspace{-0.5in}
% \includegraphics[height=1.75in]{images/glamwomen-noreferer}
\caption{A server customizes its response to a browser request by first inspecting the HTTP 
Referer field. The server returns an advertisement when the Referer field is properly set. 
Any telemetry that accompanies an ad campaign will report a page location that 
suggests the creative rendered alongside a story about home decorating projects hosted on {\tt\url{glamwomen.com}}.  
Figure~\ref{fig:watch-series-to-highspeedtesting-emulse-mensstylebook-zoom-edits} shows
a screen capture of a similar scheme.}
\label{fig:glam_ref}
\end{figure}

Inspection of panelist data coupled with a manual review of this instance shows that the sequence of requests occurs within the an iframe that is hosted on a third-party domain, \mbox{\tt\url{wwwpromoter.com}}.  Other domains that exhibit a similar URL structure and functionality are {\tt{\url{tripandleisure.com}}} and {\tt\url{quickcookingguide.com}}. Panelist data dating from May 27, 2015 shows 38K requests to these domains (recall that panelist data, while a rich and detailed data source, is but a small sample of worldwide traffic). During November 2016, the third-party domain  {\tt\url{wwwpromoter.com}} and the domain {\tt\url{tripandleisure.com}} are still in operation. A new domain, \mbox{\tt{\url{fitnessrestored.com}}}, is currently in service and  handles 36K daily requests from panelists. % Laundered telemetry that attributes ad traffic to  \mbox{\tt{\url{fitnessrestored.com}}} new domain may be triggered by visiting URLS hosted on either {\tt\url{xmovies8.tv}} and {\tt{\url{vodlocker.lol}}}. These domains purport to serve copyrighted video content.

% The code that inspects the ads context is associated with a video ad. The staging URL was never reported by the campaign telemetry. As a result, to understand how this scheme functions requries a different view of traffic.

% The feature that enabled discovery was  that campaign telemetry indicated that ads were rendered within the DOM as a sibling to the primary page content. This structure is highly unusual as it opens the publisher to the risk that the page content may be overwritten by aribtrary content. We were able to reverse-engineer and replicate the scheme based on panelist data.

%This can be seen in Figure~\ref{fig:adhex-glamwomen-census}. 

% FIXME - add a sentence or two on how we discovered this threat and which data sources were used - similar to the last paragraph on Adhexa.

% The characteristic URL that triggers the scheme is this:
% \begin{small}
% \begin{verbatim}
% tripandleisure.com/latest?category=2
% glamwomen.com/featured?category=4 
% quickcookingguide.com/quick-eats?category=3
% \end{verbatim}
% \end{small}

% curl -A 'Mozilla/5.0 (compatible; MSIE 10.0; Windows NT 6.2; Win64; x64; Trident/6.0)' 'tripandleisure.com/latest?category=2'
% curl -A '' 'tripandleisure.com/latest?category=2'
% The server response depends upon the request referrer and user agent, 
% altering its response based on these http header values:
%  \begin{figure}[ht]
%  \includegraphics[width=3.5in]{images/glamwomen-referer}
%  \includegraphics[width=3.5in]{images/glamwomen-noreferer}
%  \caption{Content returned from glamwomen URLs depends on referer of the client request}
%  \label{fig:glamwomen-refnoref}
%  \end{figure}

% \begin{small}
% \begin{verbatim}
%   GET: 'glamwomen.com/featured?category=4'
%   User-Agent: 
% RESPONSE BODY:
% <!DOCTYPE html><html><head><script>
% location.href = 
%   "http://glamwomen.com/food/\
%      4-food-proven-to-heal-a-stomach-ache";
% </script></head></html>
% 
%   GET: 'glamwomen.com/featured?category=4'
%   User-Agent: 'Mozilla/5.0 (Windows ...) like Gecko'
% RESPONSE BODY:
% <!DOCTYPE html><html><body><script>
%   var f = document.createElement("FORM"); 
%   f.method = "POST"; 
%   f.action = 
%     "http://glamwomen.com/...-up-with-bad-nutrition"; 
%   document.body.appendChild(f); 
%   f.submit();
% </script></body></html>
% \end{verbatim}
% \end{small}
% 
% \begin{small}
% \begin{verbatim}
%  POST: glamwomen.com/.../break-up-with-bad-nutrition
%  User-Agent: Mozilla/5.0 (Windows ...) like Gecko
%  Referer: http://glamwomen.com/featured?category=4
% 
% RESPONSE BODY:
% <!DOCTYPE html><html>...
% ...
%   <script async\
%   src="//delivery.roimediadigital.com/.../sat.js?v=2">
%   ...
%   comScore publisher telemetry for glamwomen
%   ...
% </script>
% \end{verbatim}
% \end{small}
% The significance here is that a GET request to the above urls returns content with the other is a POST submission.
% The POST submissioin must have the proper referrer set, or else it falls back to content. WIth the 
% referrer set, it returns

% There are at least two modes of ad deliviery. The diagram above
% illustrates one, the other mode uses Javascript to
% create a hidden form which POSTS a request to the remote server. A similar
% mechanim is employed in the mensstylebook.com case study.
% 
% We further observed an ad call to a unrelated ad server\footnote{\texttt{'http://2mdn.info/716?d=POP'}}
% was issuing redirects to these pages, selected at random:
% \begin{small}
% \begin{verbatim}
% http://quickcookingguide.com/recipe-videos
% http://glamwomen.com/featured-video
% \end{verbatim}
% \end{small}
% Each of these pages load video ads, and then
% \textit{refreshes to the other page}.
% The result is a loop between domains.

%% Surveying scale and infrastructure
%% ----------------------------------
%% One common domain: roimediadigital.com
%% This domain is anonymously owned.
%% However:
%% 
%% --> SELECT  url_refer_host,COUNT(*) AS ccc FROM panel.panel_fact WHERE recorded >= '2015-05-27' AND recorded < '2015-05-28' AND  domain_name = 'roimediadigital.com' GROUP BY url_refer_host ORDER BY ccc DESC;
%% ----------------------------------+-------
%%                                   | 25938
%%  glamwomen.com                    | 15688
%%  quickcookingguide.com            | 12867
%%  tripandleisure.com               | 11968
%%                                   | 10555
%%  optimized-by.rubiconproject.com  |  5474
%%  ebdr3.com                        |  5225
%%  www.da-ads.com                   |  4946
%%  delivery.roimediadigital.com     |  4627
%%  dspc2s.relestar.com              |  2220
%%  lax1.ib.adnxs.com                |  1850
%%  nym1.ib.adnxs.com                |  1845
%% 
%% 
%% One hypothesis that this is just ad delivery (legitimate examples, e.g. KOMO news 
%% places ads in iframes), however:
%% 
%%   1. the ad delivery is not on the top-level pages where ads are delivered
%%   2. panel traces show unusual behavior
%% 
%% Included in behavioral analysis, we have the following trace from c1=2 data:
%% 
%% -[ RECORD 22 ]-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%% c2 | 19889209
%% c7 | http://tripandleisure.com/latest?category=2
%% c4 | 
%% c9 | http://tripandleisure.com/travel/10-things-to-pack-in-your-carry-on
%% -[ RECORD 23 ]-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%% c2 | 19889209
%% c7 | http://glamwomen.com/health/choose-the-right-shoes-for-your-workout-routine
%% c4 | 
%% c9 | http://tripandleisure.com/culture/souvenirs-to-avoid-purchasing
%% -[ RECORD 24 ]-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%% c2 | 19889209
%% c7 | http://glamwomen.com/health/choose-the-right-shoes-for-your-workout-routine
%% c4 | 
%% c9 | http://tripandleisure.com/culture/souvenirs-to-avoid-purchasing
%% 
%% Google Adsense unifiers: ca-pub-2977585071826906
%%   glamwomen.com
%%   tripandleisure.com
%%   quickcookingguide.com
%%   culturemagnet.com (some similarity to trendingwoman.com)
%%   techhalt.com	 (this and 9680020357712058)
%%   highspeedtesting.com
%% 
%% Google Adsense unifiers: ca-pub-1685755517310026
%%   womenemag.com
%%   femaleinsider.com
%%   1000bites.com
%% 
%% Adsense: ca-pub-8918970543424762
%%   hongkiat.com
%%   whyresearch.com
%% 
%% Adsense: ca-pub-0823630334215913
%%   loveofcrochet.com
%% 
%%   Same UA:2024191
%% 
%% 
%% Characteristics: glamwomen.com
%% ----------------------------------
%% ${DOMAIN_NAME}/${WORD}?category=${INTEGER}
%% glamwomen.com/featured?category=2
%% the image glamwomen.com started at 
%% 
%% glamwomen.com/featured?category=2 -> 
%% glamwomen.com/living/signs-that-your-significant-other-is-cheating-on-you ->
%% http://www.nxsrv1.com/ads?key=f50c18747b98bf88c842ceae71c15781 (several of these, each loads several subframes)
%%   http://admediaco.science/?page=i&h=73e9521e93e48a95ce634ab3e8c9eca6&t=1433269982686
%% 	which load e.g.
%% 	http://ib.adnxs.com/ttj?id=4613956&referrer=http%3A%2F%2Fwww.motorauthority.com
%% 
%% See glamwomen.com_adnxs_bad_referer_all_from_category_str.png
%% 
%% This redirects to a page:
%% 
%% Unusual redirect:
%% glamwomen.com/featured-video eventually redirects to quickcookingguide
%% Jeff-Kline-MacBook-Pro:DomainLaundering jeffkline$ curl -vvv 'http://2mdn.info/716?d=POP'
%% *   Trying 199.19.78.242...
%% * Connected to 2mdn.info (199.19.78.242) port 80 (#0)
%% > GET /716?d=POP HTTP/1.1
%% > Host: 2mdn.info
%% > User-Agent: curl/7.42.1
%% > Accept: */*
%% > 
%% < HTTP/1.1 303 See Other
%% < Server: nginx
%% < Date: Mon, 01 Jun 2015 22:11:14 GMT
%% < Transfer-Encoding: chunked
%% < Connection: close
%% < Location: http://glamwomen.com/featured-video
%% < Expires: Mon, 01 Jun 2015 22:11:13 GMT
%% < Cache-Control: no-cache
%% < 
%% * Closing connection 0
%% Jeff-Kline-MacBook-Pro:DomainLaundering jeffkline$ curl -vvv 'http://2mdn.info/716?d=POP'
%% *   Trying 199.19.78.242...
%% * Connected to 2mdn.info (199.19.78.242) port 80 (#0)
%% > GET /716?d=POP HTTP/1.1
%% > Host: 2mdn.info
%% > User-Agent: curl/7.42.1
%% > Accept: */*
%% > 
%% < HTTP/1.1 303 See Other
%% < Server: nginx
%% < Date: Mon, 01 Jun 2015 22:11:16 GMT
%% < Transfer-Encoding: chunked
%% < Connection: close
%% < Location: http://quickcookingguide.com/recipe-videos
%% < Expires: Mon, 01 Jun 2015 22:11:15 GMT
%% < Cache-Control: no-cache
%% < 
%% * Closing connection 0
%% 
%% 
%% Characteristics: tripandleisure.com
%% ----------------------------------
%% Characterized as 'mode media' for simlar strcture to quickcookingguide
%% tripandleisure.com/latest?category=1
%% 
%% Characteristics: quickcookingguide.com
%% --------------------------------------
%% This is characterized as 'mode media' because:
%% 
%% Jeff-Kline-MacBook-Pro:mode jeffkline$ for f in glamwomen.com quickcookingguide.com quickmensguide.com citybartender.com highspeedtesting.com alltraveldaily.com diybaker.com diyfoodvids.com elegantrecipes.com hometechproducts.com; do dig ${f} | grep IN | grep -v '^;'; done
%% glamwomen.com.		103	IN	A	74.81.68.2
%% quickcookingguide.com.	189	IN	A	66.85.76.202
%% quickmensguide.com.	189	IN	A	162.220.112.18
%% citybartender.com.	189	IN	A	184.174.120.90
%% highspeedtesting.com.	190	IN	A	162.220.114.231
%% alltraveldaily.com.	190	IN	A	184.174.120.93
%% diybaker.com.		189	IN	A	104.28.10.33
%% diybaker.com.		189	IN	A	104.28.11.33
%% diyfoodvids.com.	189	IN	A	184.174.120.169
%% diyfoodvids.com.	189	IN	A	184.174.120.84
%% elegantrecipes.com.	189	IN	A	184.174.120.99
%% hometechproducts.com.	189	IN	A	184.174.120.103
%% hometechproducts.com.	189	IN	A	184.174.120.187
%% Jeff-Kline-MacBook-Pro:mode jeffkline$ for f in ads.glamwomen.com ads.quickcookingguide.com adserver.quickmensguide.com adserver.citybartender.com adserver.highspeedtesting.com adserver.alltraveldaily.com adserver.diybaker.com adserver.diyfoodvids.com adserver.elegantrecipes.com adserver.hometechproducts.com; do dig ${f} | grep IN | grep -v '^;'; done
%% ads.glamwomen.com.	111	IN	A	184.174.122.30
%% ads.quickcookingguide.com. 111	IN	A	184.174.122.30
%% adserver.quickmensguide.com. 111 IN	A	184.174.122.30
%% adserver.citybartender.com. 112	IN	A	184.174.122.30
%% adserver.highspeedtesting.com. 112 IN	A	184.174.122.54
%% adserver.alltraveldaily.com. 112 IN	A	184.174.122.30
%% adserver.diybaker.com.	112	IN	A	184.174.124.163
%% adserver.diyfoodvids.com. 112	IN	A	184.174.122.30
%% adserver.elegantrecipes.com. 112 IN	A	184.174.122.30
%% adserver.hometechproducts.com. 112 IN	A	184.174.122.30
%% 
%% Some of the ips (as of 2015/5/18):
%% 184.174.122.30
%% 184.174.124.166
%% 184.174.124.163
%% 
%% And the domains:
%% adserver.easygoodhealth.com (proxy)
%% adserver.1000bites.com (proxy)
%% adserver.alltraveldaily.com (proxy)
%% adserver.rawdaily.com (proxy)
%% adserver.diyfoodvids.com (proxy)
%% adserver.recipechart.com (proxy
%% adserver.worldtotravel.com (proxy)
%% adserver.diybaker.com (proxy)
%% adserver.trendingwoman.com (proxy)
%% adserver.mensstylebook.com (proxy)
%% adserver.quickmensguide.com (wwwpromoter.com, WJONES@WWWPROMOTER.COM)
%% adserver.citybartender.com (proxy)
%% adserver.hometechproducts.com (wwwpromoter.com, WJONES@WWWPROMOTER.COM)
%% adserver.streetzsavvy.com (proxy)
%% adserver.whyresearch.com (proxy)
%% adserver.moviesland.com (proxy)
%% adserver.femaleinsider.com (proxy)
%% adserver.ie-games.com (proxy)
%% adserver.smackchow.com (proxy)
%% adserver.highspeedtesting.com (proxy)
%% adserver.elegantrecipes.com (proxy)
%% yieldmanager.com (proxy)
%% 
%% 


==> mitigation.tex <==
The scale and diversity of the ad ecosystem including the variety of ways in 
which information flows between entities makes direct detection of placement 
laundering challenging.  The variety of methods employed in the case studies of 
Section~\ref{sec:cs} suggest that a variety of detection methods is required to 
accurately detect laundering.  Unfortunately, our efforts at automating detection methods 
thus far have been prone to false-positives. Reasons for this are described 
below.  We have settled on a more limited aim, namely a semi-supervised approach 
which, with a fair degree of accuracy, highlights candidates for laundering.

% We rely on web server logs and panel records that are a dim reflection of ground truth. 
\subsection{Challenges of Detection}
Automated detection seems a straightforward task: one simply 
reconciles campaign data with publisher data. Specifically, one
identifies attributed impressions served to a user and asks whether the user visited 
the domain of attribution at some recent earlier time.  False positive detections can occur in at least four ways.

First, groups of domains can be synonyms for the same service.  A popular email portal operated by Microsoft uses 
the domains \url{outlook.com}, \url{live.com}, and \mbox{\url{hotmail.com}}. A user visiting one of these domains can have ads legitimately attributed to any other. 
Similarly, ads hosted on \mbox{\url{realtor.com}} may be legitimately attributed to \mbox{\url{move.com}}.  It may be possible to track these relationships in an automated way, but 
the publishing business is very dynamic and domain names are constantly changing affiliations. 

Second, user behavior can cause false positive detections. For example, if a user loads a publisher's page in a background tab, the associated ad impressions might be served minutes or even hours later.  
It is therefore necessary to define the notion of a user session ({\em i.e.} the time between publisher visit and the attributed impression).  This has been useful to faciliate manual investigations, but it is still very much a manual review process.

Third, campaigns can have {\em ad-hoc} attribution. One example of this is ads served on the video sharing site, \mbox{\url{dailymotion.com}}. We observed
ad campaigns attributed to 
\mbox{\url{dailymotionwomen.com}}, \mbox{\url{dailymotionkia2.com}} and 
\mbox{\url{dailymotionwomen2549groupm.com}}. None of these domains resolve to IP 
addresses. But based on a review of panel data, we believe that 
the incorrect domain labels  are  basically accurate representions of the ad placements.

Finally, a publisher may not comprehensively deploy Javascript telemetry tags across all of it's pages. 
Untagged pages can serve ads that do not have a corresponding record in the publisher census data.

False negative detections can also occur. A false negative occurs when an 
ad call looks exactly like a visit to a publisher's page. Indeed, the case 
studies ``Glamwomen'' and ``bimage'' match this description. 

One fruitful source of true positive detections has relied on anomalies within {\em invalid traffic}.
Invalid traffic is a special label assigned to traffic that has no value to legitimate ad ecosystem constituents. This label is the 
end result of a proprietary ``filtering" process that is applied to all census 
and ad campaign traffic by comScore.  The theory behind invalid traffic and the 
process that assigns the label is beyond the scope of the present discussion. Surprisingly,
misattributed impressions are not necessarily invalid so this approach requires nuance.

Again, it seems straightforward to generate a list of high quality publishers and monitor this list for spikes in invalid traffic.
Unfortunately, the nature of the digital publishing business means that high 
quality publishers occasionally do experience spikes in invalid traffic. These 
spikes may have other causes such as telemetry errors or business relationships 
with disreputable traffic generators. Still, this approach can work. The AdHexa 
case study was discovered with a version of this general approach. 

% this requires a simultaneous and coordinated records of the impression measured 
% at the publisher and at the ad creative.

% This view is available from panel data and a partial view is provided by a combination of census and ad tag data.   This allowed us to implement detection methods based on different types of data.  As with any fraud detection method, our goal is to identify this behavior automatically and with high accuracy.  However, the scale of data and complexities of the mechanisms used by fraudsters complicate the problem.  
% 
%This view can be acquired in two ways: by instrumenting a broad range of individual browsers and recording their web-based activity or by instrumenting a broad set of ad campaigns and publishers' web sites.  Fortunately, both types are available from our data provider.  This allowed us to implement detection methods based on both types of collection methods. We describe below observations based on these implementations. The goal was to highlight instances where placement laudering {\em may} be occurring with enough accuracy so that manual review is a practical next step. 

% A discussion at the end of this section describes how these methods and their data sources can be combined with so-called {\em invalid traffic} to make a positive identification of placement laundering.  {\em Invalid} is a special label assigned to traffic that has no value to legitimate ad ecosystem constituents. This label is the end result of a proprietary ``filtering" process that is applied to all census and ad campaign traffic by comScore.  The theory behind invalid traffic and the process that assigns the label is independent of the present discussion. In fact, misattributed impressions are not necessarily invalid. However, we observe that laundering appears to be correlated with invalid traffic.
\subsection{Panel traffic analysis}
\label{sec:panelanalysis}
%This approach is based on a comprehensive view of all HTTP/HTTPS activity on the web browser's host machine. This is made possible when panelists (opt in participants) install specialized software on their systems that reports to a central server operated by \comscore.  Reports include all publisher and ad requests.  A more complete description is in Section \ref{sec:panelist}

%The body of active comScore panelists are the source of roughly 80 million records per hour, or about 2 billion panelist records per day.  Although this data source is just 1/10 the size of the data sources used in the JavaScript-based method described above, the data contained in this set is much richer and has higher fidelity. For example, panelists are identified by a unique machine identifier even if their browser rejects cookies. 
%Additionally, process name and process identifier are recorded.
Panel data provides a nearly complete view of an individual machine's web 
browsing activity.
Although this data source is a fraction of the size of the census and other data 
sources, panelist data is much richer. For example, panelists are identified by a unique 
machine identifier even if their browser rejects cookies.  Panel data also records
the process name that initiated each HTTP request. This is useful in identifying traffic generated by malware, for example.  As 
a result of its richness, this data can provide strong evidence of misattribution by reviewing 
the domains visited and attribution attempted across time. It does not require 
publisher or campaign participation. 

In September 2015, we searched panel traffic for ads that were requested by adware processes that also had human readable attribution in the request. 
We identified one panelist with over 500 misattributed impressions during one hour.  This web client presented 
two user agent strings representing Chrome and Internet Explorer. 

Based on the traffic associated with this panelist's instance of adware, we believe this software is capable of
rendering both video and display advertising impressions. A large portion of 
traffic generated by this process attributed the impressions to a static list of 
about 50 domains.  The sequence of ad requests repeated every 22 hours over the course of three days' worth of observations.
None of the domains of attribution were observed as part of the user's recent browsing behavior. A
subset of domains seen in this instance is shown in Figure \ref{fig:paneltrace}. 
\begin{figure}[tp]
% panel machine_id 191747934 on 9/15/2015
% \vspace{-1.25in}
% \includegraphics[width=3.25in]{{images/playthru}.pdf}
% \caption{The number of ads with incorrect attribution served during one hour on one panelist's machine. Malware is preconfigured to use 52 different domains during the course of a periodic cycle. A total of 501 impressions were identified by the panel-based methodology.}
\begin{verbatim}
...
00:44:33.718	salon.com
00:44:39.811	games.pch.com
00:44:41.932	seat61.com
00:44:48.971	huffingtonpost.co.uk
00:44:51.338	adserver.popyard.com
00:44:52.081	charter.net
00:44:52.994	dinakaran.com
00:45:51.902	tv.sohu.com
00:45:52.607	littlethings.com
...
\end{verbatim}
\caption{Each record above displays a timestamp and the attempted attribution of impressions generated by malware running on one panelists machine during September 2015. Each line represents an ad call to a particular ad exchange.  No HTTP requests went from this machine to any of domains listed above during the period of observation. The malware paused for 22 hours before resuming the same activity. }
\label{fig:paneltrace}
\end{figure}

We have developed a general algorithm that identifies candidate panelist machines that have may have been served laundered advertisements.
The algorithm consists of the following steps: 
\begin{enumerate}
\item identify all attributed ads served to every panelist's machine during one day
\item identify publishers visited by each panelist machine during one day
\item identify the domains that with the largest fraction of attributed ads with missing publisher visits
\item select those panelist machines that were engaged in the most active mis-attributed instances.
\end{enumerate}
The final step is a manual review of traffic from several of the candidate machine identifiers.  This manual review can involve visiting URLs in the panelist machine records, inspecting panelist logs for known signs of malware and looking for evidence that suggests a false positive.
\subsection{Applications of JavaScript telemetry}
\label{subsec:jsdetect}
We have applied data acquired from JavaScript telemetry deployed on 
publisher websites (the publisher census) and alongside advertising campaign 
creatives (ad tags) in two ways. First, we have used it to explore the impact 
of laundering instances that have been positively identified.  Second, this
data is ingested by the invalid traffic processes and invalid traffic has 
been useful to identify instances of laundering.

In each of the case studies discussed below, we were able to identify characteristics 
that isolate the impacted traffic. For example, in the case 
of Adhexa, the characteristic was ads served on a particular ad exchange and 
associated with a small set of account identifiers.  

% JavaScript telemetry typically tracks individuals by attempting to setting 
% cookies on the browser. Assuming a cookie is set, the same cookie is passed in 
% both publisher and ad traffic streams.  Theoretically then, one should be able to compare a user's browsing behavior against 
% ads that were served to the user and attributed to particular domains.  
% 
% But this is difficult in practice.  Even assuming that a broad slice of publisher traffic is available for inspection, 
% some publishers instrument just a small subset of their pages. This can cause ads to be served and attributed correctly without corresponding publisher telemetry. The result can be a significant source of false positives.
\subsection{Crawling to measure frame depth}
A feature common to several instances of laundering is a large number of nested iframes.
Using the methodology described in Section~\ref{sec:panelanalysis}, we 
identify panelist machines engaged in placement laundering and randomly sample 50,497 URLs from these machines' daily 
activity. Of this sample, 6,139 URLs had iframe structure. We also sample 6,485 URLs from the general panel population's daily activity, of which 660 had iframe structure.  
We crawl these urls and measure the maximum frame depth of each.  Our hypothesis is that the maximum frame depth of the 
URLs of the tainted population would tend to skew larger than frame depth of URLs 
taken from the general set of panel data. Figure~\ref{fig:urlcomp} shows that, 
indeed this is the case.  A maximum of 11 iframe nestings is observed in the 
tainted population and, generally, the portion of large frame depths is larger 
in the tainted population's URLs. 
\begin{figure}[tp]
\hspace{-0.25in}\includegraphics[width=3.25in]{{images/percentURLs_panel_analysis}.pdf}
\caption{Nesting of iframes is associated with several different instances of 
laundering. The above compares maximum frame depth of URLs visted by panel 
machines engaged in laundering (light gray) against the general population's 
frame depth (dark gray).  The ``laundering'' population's set of URLs skew 
towards larger maximum iframe depth.}
\label{fig:urlcomp}
\end{figure}

% Census and ad tags report telemetry in different ways. Thus, if a tag reports its location is on a publisher's site, it is 
% still possible to determine whether the record was called by an ad or by a user's visit to the publisher.
% The ``bimage'' case study was first identified by looking at outliers in ad traffic. The domains The set of similar domains credited with a large volume of video ads all
% had paths in the attribution appeared to be directly on the publisher page. 

% The ``adhexa'' case study was first identified by reports of invalid traffic on well-known high-reptutaion domains.  The ``bimage'' domains were first 

% The JavaScript code that is deployed by each publisher and the ad creative instructs the web browser to request a pixel from a server operated by comScore.  The pixel request either includes a cookie in the HTTP header or, if it does not, then the server responds with a new cookie.  Ideally users whose browsers accept cookies are uniquely identifiable.

% We treat each hour of the day separately and assume it is fixed. For each unique identifier (UID - cookie) observed within an hour, we construct two lists. First, we construct a trace of publisher domains that the UID visited.  Only domain-level information is used. Domains are normalized using information from  \url{https://publicsuffix.org/}.  Next, for each impression served to the UID we construct a list of domains that those impressions were attributed to.  Only domains that are currently deploying the publisher JavaScript tag are considered.  Finally, we identify attributed to domains which do not have a corresponding visit to the domain.  This method has the property that any page view on a publisher domain ``counts'' even if it was unassociated or came after a laundered placement.

% A simplified model can help elucidate the asymmetric roles of the two lists.  Consider  matrices $a\coloneqq(a_{ud}) $ and $p\coloneqq (p_{ud})$ where users are indexed by $u$, domains by $d$ and
% \begin{eqnarray*}
% {p}_{ud} & \coloneqq & \mathrm{count\ of\ visits\ by\ }u\mathrm{\ to\ domain\ }d\\
% {a}_{ud} & \coloneqq & \mathrm{count\ of\ impressions\ served\ to\ }u\mathrm{\ attributed\ to\ }d
% \end{eqnarray*}
% Most users visit a relatively small number of distinct domains in a given hour. Thus, matrices $a$ and $p$ are sparse integer-valued matrices.  The matrix $(a-p)_+$ is supported on users $u$ who had a surplus of impressions attributed to domain $d$.   The data shown in Figure~\ref{fig:slashdot-komonews} represents the sums over selected columns (domains) of $(a-p)_+$.  Sums over rows can highlight users with a large number of misattributed ads. 
% 
% Next, we turn to ad-campaign data where creatives are attributed to specific domains. We only consider records where both the domain is a census domain and the web browser submits a cookie.
% We then construct for each UID a domain list.  Given the lists of census uids and ad-uids, they are joined. 
% Any domain in the ad-list without a corresponding census ping counts as a candidate for placement laundering.

% A view of identified volume traffic over time impacting three selected domains are shown in Figure~\ref{fig:slashdot-komonews}. The figure illustrates that volume can change over the course of a single day, can end abruptly and can resume after pauses.
% 
% \begin{figure}[ht]
% \hspace{-0.5in}
% \includegraphics[width=4.0in]{{images/slashdot-komonews}.pdf}
% \caption{View over time of unmatched impressions impacting three prominent domains during the hours starting 00:00UTC and 12:00UTC over ten consecutive Fridays. We believe that none of the domains shown here had any association with the traffic represented.  Thus, this is a signal for placement laundering.}
% \label{fig:slashdot-komonews}
% \end{figure}

% The general method can highlight genuine laundering, though it also suffers from several known sources of false positives. If a user visits a domain during the final seconds of the one hour and the ad impressions are served during the successive hour, it will result in a gap in the record. This 
% risk can be reduced by shrinking the time window that informs the ad traffic attribution list (the matrix $a$).  Next, if the number of ad-tags on any one publisher is larger than one, the domain will exhibit a surplus of ad tags across all UIDs. This can be addressed by filtering out those entities or by applying other processes to normalize the data.  Other sources of false positives include errors or anomalies in tag deployment and unusual browser behavior.

% We process this data on a cluster running the Mapr version of Apache Hadoop.  The process ingests a volume of 200 million ad impressions per hour, about 5 billion per day. The publisher page view count is 600 million per hour, about 15 billion per day.  
% \subsection{A hybrid analysis, invalid activity and validating results}
% 
% Accurate identification of invalid traffic is a major concern to publishers and advertisers.  comScore uses a variety of proprietary methods to identify invalid traffic.  We use the labeled traffic from the panel as the starting point for forensic investigations.  Although publisher attribution does not play a role in the identification of invalid traffic, many of the instances of placement laundering that we have identified have been correlated with invalid traffic.
% 
% %As part of its f, comScore maintains a set of processes which identify traffic that is deemed without value. The process is known to be conservative in the sense that there are large costs incurred if organicly-driven human activity is mistakenly labeled invalid.
% 
% [FIXME - not sure how much this example helps...]  We illustrate the discussion above using two examples of activity observed on komonews.com.  Of the 10,098 misattributed impressions [FIXME - how were they misattributed?] on August 14, 2,371 were flagged as invalid.  For comparison, a random sample of records chosen from this data stream has about 3.0 percent labeled invalid. 
% 
% [FIXME - I don't understand this example either...]  For the komonews.com traffic on this same day, 501 of the 8,885 were flagged as invalid, or 5.6 percent.  The account identifier and ad exchange were constant across these impressions.   A manual review other activity associated with identifier found over 35,000 ad impressions attributed to six domains. Unusually, each record had the HTTP Referrer field set to the appropriate domain. Despite this, as a group, these impressions exhibited other characteristics more consistent with invalid traffic.  
% 
% Inspection of the client-side view panelist data suggests that malware was responsible for this traffic.
% We identified a process called `gammaqdvd\_64' which issues requests to the appropriate ad exchange with attribution set in the ad call and also sets the Referrer field of the HTTP request.
% The set of domains, account identifiers  and other attributes found in the panelist stream generated by malware is consistent with the observed attributes found in the JavaScript data stream.

% Laundered impression is not {\em a priori} invalid activity. Invalid activity The two are correlated, however.
% FIXME: new data for this.

% ------------------------------------------------------------------------
% url_idc           | vRRPbDTX4R5V3NpPpX0H3d
% domain_name       | adnxs.com
% url_host          | ib.adnxs.com
% url_dir           | /
% url_page          | tt
% recorded          | 2015-08-14 15:29:06.058
% sequence          | 52
% browser_ip1       | 98
% browser_ip2       | 115
% browser_ip3       | 118
% browser_ip4       | 8
% useragent         | Mozilla/4.0 (compatible; MSIE 7.0; Windows NT 6.2; WOW64; Trident/7.0; .NET4.0E; .NET4.0C; .NET CLR 3.5.30729; .NET CLR 2.0.50727; .NET CLR 3.0.30729)
% language          | en-us;en;q
% mimetype          | text/html
% method_id         | 1
% reply_code        | 302
% cookie_1          | 
% cookie_2          | proc=10816;app=gammaqdvd_64.exe;cl=0;rip=68.67.153.5
% ac_tag            | 
% source            | 3
% trackfile         | 20150814_15_ia8cid03_
% browser_idc       | M125ESQvNxApaaMxcVPOPN
% time_id           | 5705
% ss2k              | 492967746
% url_refer_domain  | komonews.com
% url_refer_host    | www.komonews.com
% url_refer_dir     | /
% url_refer_page    | /
% pageview_flag     | 3
% attribute_id      | 0
% query_string      | /tt?id=4591592&cb=5031&referrer=www.komonews.com
% pli_query_data    | /
% pli_post_data     | /
% browser_type      | 60006713
% person_id         | 
% language_id       | 0
% html_title        | 
% postdata          | 
% machine_id        | 176769208
% house_id          | 65645077
% browser_window_id | 10816
% html_form_fields  | 
% refer_qs          | /
% pattern_id        | -6410898
% 


% Details: show detection, result, ad call of same event.

% Other methods:

%The javascript-based method requires having a tag on a publisher's web site and a tag deployed with a campaign for ad telemetry.
%This attempts to associate publisher activity with attempts to attribute ads to the publisher.
%One can do this by observing web browser traffic directly or associate publisher data with ad addtribution indirectlywith ad addtribution indirectly

%The second method is to inspect client traffic directly, and associate ads attributed to publishers directly with publishers. The method here
%identifies ads and their publisher attribution and then identifies the gaps in the user's history.

%The first method requires partnerships with publishers to deploy the tag on their pages and sufficient coverage of deployment. The second method offers a comprehensive view of a small subset of traffic.

%It is possible to escape detection with direct methods simply because prominent domains are very popular and it is likely that a large base of users will have visited such sites.

% Less formal methods are based on traffic anomalies, but these require manual investigation.  In particular, looking for attributed ads in invalid traffic Invalid traffic can often be trace in panelist data, and a call-by-call trace can be performed to idetify the cause of the recorded event. Another method identifies nearly-simultaneous attribuatble ads delivered to the same client during a short span of time. Typically once an event like this is discovered, there are many such examples sharing traits such as ad exchange, account id and domain list.

% One other method


